A parallel-in-time collocation method using diagonalization: theory and implementation for linear problems

We present and analyze a parallel implementation of a parallel-in-time collocation method based on $\alpha$-circulant preconditioned Richardson iterations. While many papers explore this family of single-level, time-parallel "all-at-once" integrators from various perspectives, performance results of actual parallel runs are still scarce. This leaves a critical gap, because the efficiency and applicability of any parallel method heavily rely on the actual parallel performance, with only limited guidance from theoretical considerations. Further, challenges like selecting good parameters, finding suitable communication strategies, and performing a fair comparison to sequential time-stepping methods can be easily missed. In this paper, we first extend the original idea of these fixed point iterative approaches based on $\alpha$-circulant preconditioners to high-order collocation methods, adding yet another level of parallelization in time "across the method". We derive an adaptive strategy to select a new $\alpha$-circulant preconditioner for each iteration during runtime for balancing convergence rates, round-off errors, and inexactness of inner system solves for the individual time-steps. After addressing these more theoretical challenges, we present an open-source space- and time-parallel implementation and evaluate its performance for two different test problems.

==> todo.tex <==
- check table 1, stol for adv3 was 1e-14 not
- m0 in table 1 was tend
- ddnt start with initial guess with u0, I tihnk
- tau and tau tilde are wrong

DONE
====
** roundoff error analysis: "In order to figure out the round-off error we have to do that and that. Similar analysis exits [1,2,3], but ..." 
** are the comments in the pseudo code fine? YES, now they are
** add that we use speedup as a measure...
** say that comparing to other methods is too much work, it is for future work. Maybe cite slw's paradiag paper, second paper here: https://parallel-in-time.org/methods/paradiag.html. he compares it there but also just uses euler and also a direct solver.
** comment for GMRES people, what?
** change title?

